Joint Information Freshness and Completion Time Optimization for Vehicular Networks

The demand for real-time cloud applications has seen an unprecedented growth over the past decade. These applications require rapidly data transfer and fast computations. This paper considers a scenario where multiple IoT devices update information on the cloud, and request a computation from the cloud at certain times. The time required to complete the request for computation includes the time to wait for computation to start on busy virtual machines, performing the computation, waiting and service in the networking stage for delivering the output to the end user. In this context, the freshness of the information is an important concern and is different from the completion time. This paper proposes novel scheduling strategies for both computation and networking stages. Based on these strategies, the age-of-information (AoI) metric and the completion time are characterized. A convex combination of the two metrics is optimized over the scheduling parameters. The problem is shown to be convex and thus can be solved optimally. Moreover, based on the offline policy, an online algorithm for job scheduling is developed. Numerical results demonstrate significant improvement as compared to the considered baselines.

==> proof_2ndQPois.tex <==

\section{Shifted Exponential Service Time Leads to Output Poisson Process \ref{2ndQPois}}
We note  that the arrivals at the second queue in  two $M/M/1$ tandem networks are Poisson is well known in the queuing theory literature \cite{gross011}. The service distribution of the first queue in this paper is a shifted exponential distribution. We note that the deterministic shift also does not change the distribution since the number of arrivals in any time window in the steady state will be the same. Thus, the arrival distribution in the second queue will still be Poisson. 

==> proof_A.tex <==
\section{Proof of Theorem \ref{theo1}} 

The proof of this theorem relies on the concept of Adjacent Pairwise
Interchange (API) on jobs. Since the proof of this theorem follows trivially from the proof of Theorem 11.3.1 in \cite{pinedo2016scheduling}, we refer the interested reader to the book in \cite{pinedo2016scheduling}, page $301$, for detailed treatment of this.

==> proof_B.tex <==
\section{Proof of Theorem \ref{AoI_j}}

We start by noting that the waiting time
of job $j$ in the computing phase before processing does not count to the AoI since the most recent information will be used once a task has been placed for execution. Thus, only the computing service time, waiting time in the networking queue, and service time of networking will contribute to the AoI. Since the age of job $j$ is $1/\mu_j$, the age increases at its current age $1/\mu_j$ by the amount of processing times in the computing service stage and the additional time incurred by networking phase. By averaging over the choice of VM, the statement of the theorem in  \eqref{AoI_{j}2} follows.   

==> proof_C.tex <==
\section{Proof of Theorem \ref{C_j}}


We note that the expected release (arrival) time of a job $j$ is $\frac{1}{\lambda_j}$. This time also represents the earliest time, on expectation, that a job $j$ can be available to start processing. Clearly, the amount of work still to be done for a job $j$ to be complete increases at a release time by the amount of processing times in both computing phase and networking phase. By averaging over the choice of the VM and ignoring the term $(1/\lambda_{j})$ since its is fixed and thus cannot be optimized, we can find the expected completion time of a job $j$ as below
\begin{align*}
\mathbb{E}\left[\boldsymbol{C}_{j}\right]=\sum_{v=1}^{V}\left[p_{j,v}\left(\mathbb{E}\left[\boldsymbol{W}_{1,j,v}\right]+\mathbb{E}\left[\boldsymbol{S}_{1,j,v}\right]\right)\right] \nonumber \\
+\mathbb{E}\left[\boldsymbol{W}_{2,j}\right]+\mathbb{E}\left[\boldsymbol{S}_{2,j}\right]	\label{C_{j}23}
\end{align*}
which proves the statement of the theorem. 

==> proof_D.tex <==
\section{Proof of Theorem \ref{convxOptProb}}

Since the sum of convex functions is convex \cite{boyd2004convex}, it is enough to show that:
\begin{equation}
\sum_{v}\Lambda_{v}\mathbb{E}\left[\boldsymbol{W}_{1,j,v}\right]+\sum_{v}\Lambda_{v}\mathbb{E}\left[\boldsymbol{S}_{1,j,v}\right]+  \sum_{j}\frac{\lambda j}{\lambda}\mathbb{E}\left[\boldsymbol{W}_{2,j}\right]\label{eqConvx}
\end{equation}
 is convex. However, the last term is independent on $\boldsymbol{p}$ and thus can be ignored. Further, since  $\Lambda_{v}$ is a linear function of $\boldsymbol{p}$, it is enough to prove the convexity with respect to $\Lambda_{v}$. It is easy to show that the second term  in \eqref{eqConvx} is linear functions in $\Lambda_{v}$ and thus convex. For the first term in \eqref{eqConvx}, after simplifying the term, it can be written as
\begin{align}
\frac{\sum_{j}p_{j,v}\lambda_{j}\left(\beta_{v,j}^{2}+\beta_{v,j}+\frac{\beta_{v,j}+2}{\alpha_{v,j}}\right)}{1-\sum_{j}p_{j,v}\lambda_{j}\left(\beta_{v,j}+\frac{1}{\alpha_{v,j}}\right)} \label{1stTerm}
\end{align}
%
%By calculating the Hessian matrix for the quantity in \eqref{1stTerm}, we can show that it is convex with respect to $\boldsymbol{p}$. Moreover, It is not that hard to see that for $j=1$ and $j=2$, the above function is convex. Using similar analogy, we can prove it for any $j\geq 2$.
Now,  we need to show that the above function is convex in $\boldsymbol{p}$. We note that the above function can be expressed as $\eta\boldsymbol{x}^{T}(\boldsymbol{I}-\boldsymbol{x})^{-1}$,
where $\eta>1$ and $\boldsymbol{x}$ is a $J$-dimensional vector. The role of $\eta$ is to capture the ratio between the two terms $\sum_{j}p_{j,v}\lambda_{j}\left(\beta_{v,j}^{2}+\beta_{v,j}+\frac{\beta_{v,j}+2}{\alpha_{v,j}}\right)$
and $\left(\sum_{j}p_{j,v}\lambda_{j}\left(\beta_{v,j}+\frac{1}{\alpha_{v,j}}\right)\right)$.
This function is jointly convex on $x_{j}$ for all $j$ if and only
if $x_{j}<1$, for all $j$, see \cite{boyd2004convex} for detailed treatment on this. In our expression, $x_{j}$ represents the load
intensity (i.e., $p_{j,v}\lambda_{j}(\beta_{j}+\frac{1}{\alpha_{j}})$)
and should be less than one for stability of the system. Thus, the
above expression is convex with respect to $\boldsymbol{p}$.
%
%
% For the last term in  \eqref{eqConvx}, we need to show that $\frac{\mathbb{E}\left[\boldsymbol{Z}_{2}^{2}\right]}{\left(1-\sum_{z=1}^{j}\rho_{z}\right)\left(1-\sum_{z=1}^{j-1}\rho_{z}\right)}
%$ is convex with respect to $\boldsymbol{p}$. This is equivalent to prove convexity for $\frac{\lambda_{j}\left(\zeta_{j}^{2}+\zeta_{j}+\frac{\zeta_{j}+2}{\gamma_{j}}\right)}{\left(1-\sum_{z=1}^{j}\rho_{z}\right)\left(1-\sum_{z=1}^{j-1}\rho_{z}\right)}
%$ with respect to $\boldsymbol{\rho}=(\rho_j,\, \forall j)$. To prove that, we first show that for $j=2$ and $j=3$, the Hessian matrix ${\bf H}$ is greater than (or equal to) zero. Then, we generalize it for any $j>3$. To do so, for $j=2$, we can write 
%
%\[
%\boldsymbol{H}_{2}=\left[\begin{array}{cc}
%\frac{2}{x^{3}y} & \frac{1}{xy^{3}}\\
%\frac{1}{x^{3}y} & \frac{2}{xy^{3}}
%\end{array}\right]
%\]
%where $x=1-\rho_1$ and $y=\rho_1-\rho_2$. Since, $\boldsymbol{H}_{2}>0$, the function is strictly convex in $x,\,y$ and thus it is jointly convex in $\rho_1$ and $\rho_2$ as both are linear transformation of $x$ and $y$. Similarly, we can show that for $j=3$
%\[
%\boldsymbol{H}_{3}=\left[\begin{array}{ccc}
%\frac{2}{x^{3}yz} & \frac{1}{x^{2}y^{2}z} & \frac{1}{x^{2}yz^{2}}\\
%\frac{1}{x^{2}y^{2}z} & \frac{2}{xy^{3}z} & \frac{1}{xy^{2}z^{2}}\\
%\frac{1}{x^{2}yz^{2}} & \frac{1}{xy^{2}z^{2}} & \frac{2}{xyz^{3}}
%\end{array}\right]
%\]
%where $x,\,y,\,z$ are linear transformation of $\rho_i,\,i=1,2,3$.  Since, $\boldsymbol{H}_{3}>0$, the function is strictly convex in $ \boldsymbol{\rho}$. Thus, this result can be generalized to any $j>3$ as we can see that the determinant is always positive for any value of $j$. This proves the statement of the theorem.
%
% 
